SpaceTime: Causal Discovery from Non-Stationary Time Series

Understanding causality is challenging and often complicated by changing causal relationships over time and across environments. Climate patterns, for example, shift over time with recurring seasonal trends, while also depending on geographical characteristics such as ecosystem variability. Existing methods for discovering causal graphs from time series either assume stationarity, do not permit both temporal and spatial distribution changes, or are unaware of locations with the same causal relationships. In this work, we therefore unify the three tasks of causal graph discovery in the non-stationary multi-context setting, of reconstructing temporal regimes, and of partitioning datasets and time intervals into those where invariant causal relationships hold. To construct a consistent score that forms the basis of our method, we employ the Minimum Description Length principle. Our resulting algorithm SPACETIME simultaneously accounts for heterogeneity across space and non-stationarity over time. Given multiple time series, it discovers regime changepoints and a temporal causal graph using non-parametric functional modeling and kernelized discrepancy testing. We also show that our method provides insights into real-world phenomena such as river-runoff measured at different catchments and biosphere-atmosphere interactions across ecosystems.

==> figs/bar/bar_lin.tex <==
\def\methods{gp-plain,gp-plain-timed, gp-plain-bins,gp-plain-bins-timed, J-pcmcmi,J-pcmcmi-timed, varLINGAM-c, varLINGAM-C}
\def\var{T}
\def\file{expres/N_6_C_1_R_2_vary_T.csv}

\def\method_names{\textbf{ours} (known regimes),\textbf{ours} (k.r.) \emph{(timed)},\textbf{ours} (5 bins),\textbf{ours} (5 bins) \emph{(timed)},JPCMCI+,JPCMCI+\emph{(timed)},VarLiNGAM-$c$,VarLiNGAM-$C$}


 
\begin{figure*}[t]
	\centering
	\begin{tikzpicture}
         \pgfplotstableread[col sep=comma]{data.csv}\csvdata
	% Boxplot groups columns, but we want rows
	\pgfplotstabletranspose\datatransposed{\csvdata} 
	\begin{axis}[   pretty boxplot regime   ]
	\def\metric{f1};
	\foreach \name in \methods{    
		\addplot+[ area legend] table %[x =\var, y=\name_\metric]
  {\datatransposed}; 
	}     
	\end{axis}
	\end{tikzpicture}		 
		\begin{tikzpicture} 
	\begin{axis}[
        pretty ybar regime,
	ylabel={TPR}
	] 
	\def\metric{tpr}; 
	\foreach \name in \methods{   
		\addplot table[x =\var, y=\name_\metric] {\file}; 
	}     
	\end{axis}
	\end{tikzpicture}
	\begin{tikzpicture}
	\begin{axis}[
        pretty ybar regime,
	ylabel={FPR},
	legend entries={\textbf{ours} (known regimes),\textbf{ours} (k.r.) \emph{(timed)},\textbf{ours} (5 bins),\textbf{ours} (5 bins) \emph{(timed)},JPCMCI+,JPCMCI+\emph{(timed)},VarLiNGAM-$c$,VarLiNGAM-$C$}, legend columns=1,
			] 
			\def\metric{fpr}; 
			\foreach \name in \methods{   
				\addplot table[x =\var, y=\name_\metric] {\file}; 
			}     
	\end{axis}
	\end{tikzpicture}   
	\caption{ 
	\label{fig:dag_search:bar_lin}  Linear, $N=6$ nodes, $C=1$ context,  $|C|=250$ samples, $R=2$ regimes per context.}
\end{figure*}

==> figs/bar/bar_nlin.tex <==
\def\methods{gp-plain,gp-plain-timed, gp-bins,gp-bins-timed, J-pcmcmi,J-pcmcmi, varLINGAM-c, varLINGAM-C}
\begin{figure*} [t]
	\centering
	\begin{tikzpicture}
	\begin{axis}[
        pretty ybar regime
	] 
	\def\metric{f1};
	\def\var{T};
	\def\file{expres/N_6_T_250_R_2_C_3_nlin.csv};
	\foreach \name in \methods{   
		\addplot table[x =\var, y=\name_\metric] {\file}; 
	}     
	\end{axis}
	\end{tikzpicture}		\begin{tikzpicture}
	\begin{axis}[
        pretty ybar regime,
	ylabel={SHD} 
	] 
	\def\metric{shd};
	\def\var{T};
	\def\file{expres/N_6_T_250_R_2_C_3_nlin.csv};
	\foreach \name in \methods{   
		\addplot table[x =\var, y=\name_\metric] {\file}; 
	}     
	\end{axis}
	\end{tikzpicture}
	\begin{tikzpicture} 
	\begin{axis}[
        pretty ybar regime,
	ylabel={TPR}
	] 
	\def\metric{tpr};
	\def\var{T};
	\def\file{expres/N_6_T_250_R_2_C_3_nlin.csv};
	\foreach \name in \methods{   
		\addplot table[x =\var, y=\name_\metric] {\file}; 
	}     
	\end{axis}
	\end{tikzpicture}
	\begin{tikzpicture}
	\begin{axis}[
        pretty ybar regime,
	ylabel={FPR}
	] 
	\def\metric{fpr};
	\def\var{T};
	\def\file{expres/N_6_T_250_R_2_C_3_nlin.csv};
	\foreach \name in \methods{   
		\addplot table[x =\var, y=\name_\metric] {\file}; 
	}     
	\end{axis}
	\end{tikzpicture}   
	\caption{ 	\label{fig:dag_search:bar_lin}  Nonlinear, $N=6$ nodes, $C=3$ contexts,  $|C|=250$ samples, $R=2$ regimes per context.}
\end{figure*}

==> figs/box/dag_timed_cps.tex <==
\def\oracles{gp-kncps/\ns,  R-pcmci-kncps/\ns, pcmciplus/\ns,  
varLINGAM-kncps/\nsvlngkncps, dynotears-kncps/\ns, cdnod-kncps/\ns} 
\def\timedoracles{gp-kncps/\ns, J-pcmci-kncps/\ns, R-pcmci-kncps/\ns, R-pcmci-kncps/\ns, 
varLINGAM-kncps/\nsvlngkncps, dynotears-kncps/\ns} 
\def\cps{gp-kndag/\ns, gp/\ns, R-pcmci/\nsrpcmci}
\def\cpsadjusted{gp-kndag/\nsgpkndagcps, gp/\nsgpcps, R-pcmci/\nsrpcmcicps}
\def\methods{gp-kncps/\ns,gp/\ns, 
J-pcmci-kncps/\ns, J-pcmci/\ns, R-pcmci-kncps/\ns, R-pcmci/\nsrpcmci,  R-pcmci-kncps/\ns, %Rpcmcikncps and PCMICIplus kncps are the same!
pcmciplus/\ns, varLINGAM-kncps/\nsvlngkncps, varLINGAM/\ns,  dynotears-kncps/\ns, dynotears/\ns, cdnod-kncps/\ns, cdnod/\ns}
\def\timedmethods{gp-kncps/\ns,gp/\ns, 
J-pcmci-kncps/\ns, J-pcmci/\ns, R-pcmci-kncps/\ns, R-pcmci/\nsrpcmci,  R-pcmci-kncps/\ns, %Rpcmcikncps and PCMICIplus kncps are the same!
pcmciplus/\ns, varLINGAM-kncps/\nsvlngkncps, varLINGAM/\ns,  dynotears-kncps/\ns, dynotears/\ns} 
\begin{figure*} [t]
	\centering 
		\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={DAG},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0,  ymax= 1.1, 
   width= 7.5cm, height=4.5cm,
			ylabel={Dir. F1}, xlabel={ }, xticklabels=none,   legend entries={} ,   
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{f1};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \methods{   
				\addplot+[ area legend, boxplot = {%
				average = auto,
				every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
			}] table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}     
		\end{axis}
	\end{tikzpicture} 
	\begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={Timed DAG}, 
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0, ymax= 1.1, width= 7.5cm, height=4.5cm,
			ylabel={TCG-F1}, xlabel={ }, xticklabels=none,legend entries={, \textbf{gp},,J-PCMCI+,, R-PCMCI,,
   PCMCI+,, VARLiNGAM,, DYNOTEARS, ,CD-NOD},legend columns=1, legend style=  {at = {(1.1, 0.9)}, anchor	= north west, font=\scriptsize}, 
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{f1-timed};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \timedmethods{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
				}] table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}     
    \addplot+[area legend, boxplot = {%
				average = auto,%
				every average/.style={/tikz/mark=diamond*,/tikz/mar
    k size =2pt},%
			}, 
			] coordinates {(0,-1)};
      \addplot+[area legend, boxplot = {%
				average = auto,%
				every average/.style={/tikz/mark=diamond*,/tikz/mar
    k size =2pt},%
			}, 
			] coordinates {(0,-1)};
		\end{axis}
	\end{tikzpicture} 
 \begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={CPS},  
			 pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={CPS-F1}, xlabel={ }, xticklabels=none,  pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-f1}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \cps{   
			\addplot+[area legend, boxplot = {%
				average = auto,%
				every average/.style={/tikz/mark=diamond*,/tikz/mar
    k size =2pt},%
			}, 
			]  table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}   
		\end{axis}
	\end{tikzpicture} 
 		\begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={Partition  },  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={ARI}, xlabel={ }, xticklabels=none, 		legend entries={ }, legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize},  
	 	pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-ari}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \cps{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
					 }]  table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}     
		\end{axis}
	\end{tikzpicture}
 		\begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={  },  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={NMI}, xlabel={ }, xticklabels=none,legend entries={gp-known dag ,\textbf{gp} , R-PCMCI},
	 	pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-nmi}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \cps{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
					 }]  table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}     
		\end{axis}
	\end{tikzpicture}  
\begin{tabular}{lll}
\scriptsize{\textbf{method}} & \scriptsize{\textbf{successful runs}}  & \scriptsize{\textbf{perfect CPS-F1}}       \\ \hline  
\scriptsize{ours}            & \scriptsize{\ns   /20}    & \scriptsize{\nsgpcps   /20}   \\
\scriptsize{ R-PCMCI }        & \scriptsize{\nsrpcmci /20 }   & \scriptsize{\nsrpcmcicps /20 }\\  
\end{tabular} 
	\caption{ 	\label{fig:dag_search:boxes} \id }
\end{figure*}


==> figs/box/dag_timed_cps_large.tex <==
\def\oracles{gp-kncps/\ns,  R-pcmci-kncps/\ns, pcmciplus/\ns,  
varLINGAM-kncps/\nsvlngkncps, dynotears-kncps/\ns, cdnod-kncps/\ns} 
\def\timedoracles{gp-kncps/\ns, J-pcmci-kncps/\ns, R-pcmci-kncps/\ns, R-pcmci-kncps/\ns, 
varLINGAM-kncps/\nsvlngkncps, dynotears-kncps/\ns} 
\def\cps{gp-kndag/\ns, gp/\ns, R-pcmci/\nsrpcmci}
\def\cpsadjusted{gp-kndag/\nsgpkndagcps, gp/\nsgpcps, R-pcmci/\nsrpcmcicps}
\def\methods{gp-kncps/\ns,gp/\ns, 
J-pcmci-kncps/\ns, J-pcmci/\ns, R-pcmci-kncps/\ns, R-pcmci/\nsrpcmci,  R-pcmci-kncps/\ns, %Rpcmcikncps and PCMICIplus kncps are the same!
pcmciplus/\ns, varLINGAM-kncps/\nsvlngkncps, varLINGAM/\ns,  dynotears-kncps/\ns, dynotears/\ns, cdnod-kncps/\ns, cdnod/\ns}
\def\timedmethods{gp-kncps/\ns,gp/\ns, 
J-pcmci-kncps/\ns, J-pcmci/\ns, R-pcmci-kncps/\ns, R-pcmci/\nsrpcmci,  R-pcmci-kncps/\ns, %Rpcmcikncps and PCMICIplus kncps are the same!
pcmciplus/\ns, varLINGAM-kncps/\nsvlngkncps, varLINGAM/\ns,  dynotears-kncps/\ns, dynotears/\ns} 
\begin{figure*} [t]
	\centering 
		\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={Runtimes},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0,  ymode = log, 
   width= 7.5cm, height=4.5cm,
			ylabel={Time (s)}, xlabel={ }, xticklabels=none,   legend entries={} ,   
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{time};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \methods{   
				\addplot+[ area legend, boxplot = {%
				average = auto,
				every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
			}] table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}     
		\end{axis}
	\end{tikzpicture}
	\begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={Timed DAG}, 
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0, ymax= 1.1, width= 7.5cm, height=4.5cm,
			ylabel={TCG-F1}, xlabel={ }, xticklabels=none,legend columns=1, legend style=  {at = {(1.1, 0.9)}, anchor	= north west, font=\scriptsize}, 
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{f1-timed};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \timedmethods{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
				}] table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}     
    \addplot+[area legend, boxplot = {%
				average = auto,%
				every average/.style={/tikz/mark=diamond*,/tikz/mar
    k size =2pt},%
			}, 
			] coordinates {(0,-1)};
      \addplot+[area legend, boxplot = {%
				average = auto,%
				every average/.style={/tikz/mark=diamond*,/tikz/mar
    k size =2pt},%
			}, 
			] coordinates {(0,-1)};
		\end{axis}
	\end{tikzpicture} 
  \begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={DAG SHD},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0,  
   width= 7.5cm, height=4.5cm,
			ylabel={SHD}, xlabel={ }, xticklabels=none,   legend entries={} ,   
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{shd};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \methods{   
				\addplot+[ area legend, boxplot = {%
				average = auto,
				every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
			}] table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}     
		\end{axis}
	\end{tikzpicture}  \begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={DAG F1},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0,  ymax= 1.1, 
   width= 7.5cm, height=4.5cm,
			ylabel={Dir. F1}, xlabel={ }, xticklabels=none,   legend entries={} ,   
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{f1};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \methods{   
				\addplot+[ area legend, boxplot = {%
				average = auto,
				every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
			}] table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}     
		\end{axis}
	\end{tikzpicture} 
 	\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={DAG TPR},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0,  ymax= 1.1, 
   width= 7.5cm, height=4.5cm,
			ylabel={TPR}, xlabel={ }, xticklabels=none,   legend entries={} ,   
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{tpr};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \methods{   
				\addplot+[ area legend, boxplot = {%
				average = auto,
				every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
			}] table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}     
		\end{axis}
	\end{tikzpicture} 
	\begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={DAG FPR}, 
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0, ymax= 1.1, width= 7.5cm, height=4.5cm,
			ylabel={FPR}, xlabel={ }, xticklabels=none,legend entries={, \textbf{gp},,J-PCMCI+,, R-PCMCI,,
   PCMCI+,, VARLiNGAM,, DYNOTEARS, ,CD-NOD},legend columns=1, legend style=  {at = {(1.1, 0.9)}, anchor	= north west, font=\scriptsize}, 
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{fpr};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \methods{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
				}] table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}     
		\end{axis}
	\end{tikzpicture} 
 \begin{tikzpicture} 
 	\begin{axis}[ 
			pretty boxplot regime, title={Cutpoint Search},  
			 pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymode = log,
			ylabel={Time (s) }, xlabel={ }, xticklabels=none,  pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{time}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \cps{   
			\addplot+[area legend, boxplot = {%
				average = auto,%
				every average/.style={/tikz/mark=diamond*,/tikz/mar
    k size =2pt},%
			}, 
			]  table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}   
		\end{axis}
	\end{tikzpicture} 
  \begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={},  
			 pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={CPS-F1}, xlabel={ }, xticklabels=none,  pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-f1}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \cps{   
			\addplot+[area legend, boxplot = {%
				average = auto,%
				every average/.style={/tikz/mark=diamond*,/tikz/mar
    k size =2pt},%
			}, 
			]  table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}   
		\end{axis}
	\end{tikzpicture} 
  \begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={},  
			 pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={CPS-Precision}, xlabel={ }, xticklabels=none,  pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-prec}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \cps{   
			\addplot+[area legend, boxplot = {%
				average = auto,%
				every average/.style={/tikz/mark=diamond*,/tikz/mar
    k size =2pt},%
			}, 
			]  table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}   
		\end{axis}
	\end{tikzpicture} 
  \begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={},  
			 pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={CPS-Recall}, xlabel={ }, xticklabels=none, legend entries={gp-known dag ,\textbf{gp} , R-PCMCI}, pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-rec}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \cps{   
			\addplot+[area legend, boxplot = {%
				average = auto,%
				every average/.style={/tikz/mark=diamond*,/tikz/mar
    k size =2pt},%
			}, 
			]  table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}   
		\end{axis}
	\end{tikzpicture} 
 		\begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={Regime- and Context Partitioning},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={ARI}, xlabel={ }, xticklabels=none, 		legend entries={ }, legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize},  
	 	pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-ari}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \cps{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
					 }]  table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}     
		\end{axis}
	\end{tikzpicture}
 		\begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={  },  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={NMI}, xlabel={ }, xticklabels=none,legend entries={gp-known dag ,\textbf{gp} , R-PCMCI},
	 	pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-nmi}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \cps{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
					 }]  table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}     
		\end{axis}
	\end{tikzpicture}  
\begin{tabular}{lll}
\scriptsize{\textbf{method}} & \scriptsize{\textbf{successful runs}}  & \scriptsize{\textbf{perfect CPS-F1}}       \\ \hline  
\scriptsize{ours}            & \scriptsize{\ns   /20}    & \scriptsize{\nsgpcps   /20}   \\
\scriptsize{ R-PCMCI }        & \scriptsize{\nsrpcmci /20 }   & \scriptsize{\nsrpcmcicps /20 }\\  
\end{tabular} 
	\caption{ 	\label{fig:dag_search:boxes} \id }
\end{figure*}


==> figs/box/old/box_lin_gauss.tex <==
\def\oracles{gp-kncps, J-pcmci-kncps, R-pcmci-kncps, R-pcmci-kncps,  
varLINGAM-kncps, dynotears-kncps, cdnod-kncps}
\def\timedoracles{gp-kncps, J-pcmci-kncps, R-pcmci-kncps, R-pcmci-kncps, 
varLINGAM-kncps, dynotears-kncps}
\def\cps{gp-kndag, gp, R-pcmci}
\def\methods{gp, J-pcmci, R-pcmci,
pcmciplus, varLINGAM, dynotears, cdnod}
\def\timedmethods{gp, J-pcmci, R-pcmci, 
pcmciplus, varLINGAM, dynotears} 
\def\nonlinear{expres/box/c_2_r_3_cps_2_n_5_t_200_d_1_i_0.5_ivs_50_f_lin_ns_gauss_hi_False.csv}
\def\id{\emph{linear, gaussian noise, mechanism changes, N5C2R2CPS1T200IV0.5}}
 %TODO show successes as a table next to CPS and next to DAG
\begin{figure*} [t]
	\centering 
	\begin{tikzpicture} 
	\begin{axis}[%legend image post style={mark=*}
		pretty boxplot regime, title={DAG, known CPS},  
		pretty enlargexlimits,  
		scatter src			= explicit symbolic,  
		cycle list name =prcl-box-time,
		pretty xlabelrot, 
		ymin = 0, ymax= 1.1,width= 6cm,height=4.5cm,
		ylabel={Dir. F1}, xlabel={ }, xticklabels=none, 
		pretty labelshift,
		] 
		% PARAMETERS
		\def\metric{f1};
		\def\var{C}; 
		\def\file{\nonlinear};  
		\foreach \name in \oracles{   
				\addplot+[ area legend, boxplot = {%
				average = auto,
				every average/.style={/tikz/mark=diamond*,/tikz/mark size=2pt},% 
			}]  table[y=\name_\metric] {\file};   
		}     
	\end{axis}
\end{tikzpicture}  
		\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={DAG},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0, ymax= 1.1, width= 6cm, height=4.5cm,
			ylabel={Dir. F1}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
			legend entries={\textbf{gp},J-PCMCI, R-PCMCI,
   PCMCI+, VARLiNGAM, DY-NOTEARS, CD-NOD}, legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, 
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{f1};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name in \methods{   
				\addplot+[ area legend, boxplot = {%
				average = auto,
				every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
			}] table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture} 
	\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={Timed DAG, known CPS},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0, ymax= 1.1,width= 6cm,height=4.5cm,
			ylabel={TCG-F1}, xlabel={ }, xticklabels=none, 
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{f1-timed};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name in \timedoracles{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
				}]  table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture}  
	\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={Timed DAG},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0, ymax= 1.1, width= 6cm, height=4.5cm,
			ylabel={TCG-F1}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
			legend entries={\textbf{gp},J-PCMCI,  R-PCMCI, 
   PCMCI+,  VARLiNGAM, DY-NOTEARS, CD-NOD}, legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, 
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{f1-timed};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name in \timedmethods{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
				}] table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture} 
 \begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={CPS},  
			 pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={CPS-F1}, xlabel={ }, xticklabels=none,  pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-f1}; 
			\def\file{\nonlinear};  
			\foreach \name in \cps{   
			\addplot+[area legend, boxplot = {%
				average = auto,%
				every average/.style={/tikz/mark=diamond*,/tikz/mar
    k size =2pt},%
			}, 
			]  table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture} 
		\begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={Partition  },  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={ARI}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
	 	%	legend entries={\textbf{gp}-kndag,\textbf{gp},R-PCMCI }, legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, , 
	 	pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-ari}; 
			\def\file{\nonlinear};  
			\foreach \name in \cps{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
					 }]  table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture}
			\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
		%	pretty ybar regime, 
			pretty boxplot regime, 
			title={Successes},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={Fract. successful runs}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
				legend entries={\textbf{gp}-kndag,\textbf{gp}, R-PCMCI
    },
    legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{valid};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name in \cps{   
				\addplot+[area legend]  table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture}
	\caption{ 	\label{fig:dag_search:boxes} \id }
\end{figure*}


==> figs/box/old/box_lin_unif.tex <==
\def\oracles{gp-kncps, J-pcmci-kncps, R-pcmci-kncps, R-pcmci-kncps,  
varLINGAM-kncps, dynotears-kncps, cdnod-kncps}
\def\timedoracles{gp-kncps, J-pcmci-kncps, R-pcmci-kncps, R-pcmci-kncps, 
varLINGAM-kncps, dynotears-kncps}
\def\cps{gp-kndag, gp, R-pcmci}
\def\methods{gp, J-pcmci, R-pcmci,
pcmciplus, varLINGAM, dynotears, cdnod}
\def\timedmethods{gp, J-pcmci, R-pcmci, 
pcmciplus, varLINGAM, dynotears} 
\def\nonlinear{expres/box/c_2_r_3_cps_2_n_5_t_200_d_1_i_0.5_ivs_50_f_lin_ns_unif_hi_False.csv}
\def\id{\emph{linear, uniform noise, mechanism changes, N5C2R2CPS1T200IV0.5}}
 %TODO show successes as a table next to CPS and next to DAG
\begin{figure*} [t]
	\centering 
	\begin{tikzpicture} 
	\begin{axis}[%legend image post style={mark=*}
		pretty boxplot regime, title={DAG, known CPS},  
		pretty enlargexlimits,  
		scatter src			= explicit symbolic,  
		cycle list name =prcl-box-time,
		pretty xlabelrot, 
		ymin = 0, ymax= 1.1,width= 6cm,height=4.5cm,
		ylabel={Dir. F1}, xlabel={ }, xticklabels=none, 
		pretty labelshift,
		] 
		% PARAMETERS
		\def\metric{f1};
		\def\var{C}; 
		\def\file{\nonlinear};  
		\foreach \name in \oracles{   
				\addplot+[ area legend, boxplot = {%
				average = auto,
				every average/.style={/tikz/mark=diamond*,/tikz/mark size=2pt},% 
			}]  table[y=\name_\metric] {\file};   
		}     
	\end{axis}
\end{tikzpicture}  
		\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={DAG},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0, ymax= 1.1, width= 6cm, height=4.5cm,
			ylabel={Dir. F1}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
			legend entries={\textbf{gp},J-PCMCI, R-PCMCI,
   PCMCI+, VARLiNGAM, DY-NOTEARS, CD-NOD}, legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, 
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{f1};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name in \methods{   
				\addplot+[ area legend, boxplot = {%
				average = auto,
				every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
			}] table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture} 
	\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={Timed DAG, known CPS},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0, ymax= 1.1,width= 6cm,height=4.5cm,
			ylabel={TCG-F1}, xlabel={ }, xticklabels=none, 
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{f1-timed};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name in \timedoracles{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
				}]  table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture}  
	\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={Timed DAG},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0, ymax= 1.1, width= 6cm, height=4.5cm,
			ylabel={TCG-F1}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
			legend entries={\textbf{gp},J-PCMCI,  R-PCMCI, 
   PCMCI+,  VARLiNGAM, DY-NOTEARS, CD-NOD}, legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, 
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{f1-timed};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name in \timedmethods{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
				}] table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture} 
 \begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={CPS},  
			 pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={CPS-F1}, xlabel={ }, xticklabels=none,  pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-f1}; 
			\def\file{\nonlinear};  
			\foreach \name in \cps{   
			\addplot+[area legend, boxplot = {%
				average = auto,%
				every average/.style={/tikz/mark=diamond*,/tikz/mar
    k size =2pt},%
			}, 
			]  table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture} 
		\begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={Partition  },  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={ARI}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
	 	%	legend entries={\textbf{gp}-kndag,\textbf{gp},R-PCMCI }, legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, , 
	 	pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-ari}; 
			\def\file{\nonlinear};  
			\foreach \name in \cps{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
					 }]  table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture}
			\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
		%	pretty ybar regime, 
			pretty boxplot regime, 
			title={Successes},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={Fract. successful runs}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
				legend entries={\textbf{gp}-kndag,\textbf{gp}, R-PCMCI
    },
    legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{valid};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name in \cps{   
				\addplot+[area legend]  table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture}
	\caption{ 	\label{fig:dag_search:boxes} \id }
\end{figure*}


==> figs/box/old/box_nlin_c1.tex <==
\def\oracles{gp-kncps, J-pcmci-kncps, R-pcmci-kncps, R-pcmci-kncps,  
varLINGAM-kncps, dynotears-kncps, cdnod-kncps}
\def\timedoracles{gp-kncps, J-pcmci-kncps, R-pcmci-kncps, R-pcmci-kncps, 
varLINGAM-kncps, dynotears-kncps}
\def\cps{gp-kndag, gp, R-pcmci}
\def\methods{gp, J-pcmci, R-pcmci,
pcmciplus, varLINGAM, dynotears, cdnod}
\def\timedmethods{gp, J-pcmci, R-pcmci, 
pcmciplus, varLINGAM, dynotears}
\def\linear{expres/box/c_3_r_2_cps_3_n_3_t_200_d_1_i_2_ivs_50_f_lin_ns_unif.csv}
\def\nonlinear{expres/box/c_1_r_2_cps_4_n_5_t_200_d_1_i_2_ivs_50_f_exp_ns_unif.csv} 
\def\id{\emph{nonlinear, uniform noise, C1R2CPS4T200IV2}}
 %TODO show successes as a table next to CPS and next to DAG
\begin{figure*} [t]
	\centering 
	\begin{tikzpicture} 
	\begin{axis}[%legend image post style={mark=*}
		pretty boxplot regime, title={DAG, known CPS},  
		pretty enlargexlimits,  
		scatter src			= explicit symbolic,  
		cycle list name =prcl-box-time,
		pretty xlabelrot, 
		ymin = 0, ymax= 1.1,width= 6cm,height=4.5cm,
		ylabel={Dir. F1}, xlabel={ }, xticklabels=none, 
		pretty labelshift,
		] 
		% PARAMETERS
		\def\metric{f1};
		\def\var{C}; 
		\def\file{\nonlinear};  
		\foreach \name in \oracles{   
				\addplot+[ area legend, boxplot = {%
				average = auto,
				every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
			}]  table[y=\name_\metric] {\file};   
		}     
	\end{axis}
\end{tikzpicture}  
		\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={DAG},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0, ymax= 1.1, width= 6cm, height=4.5cm,
			ylabel={Dir. F1}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
			legend entries={\textbf{gp},J-PCMCI, %R-PCMCI,
   PCMCI+, VARLiNGAM, DY-NOTEARS, CD-NOD}, legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, 
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{f1};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name in \methods{   
				\addplot+[ area legend, boxplot = {%
				average = auto,
				every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
			}] table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture} 
	\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={Timed DAG, known CPS},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0, ymax= 1.1,width= 6cm,height=4.5cm,
			ylabel={TCG-F1}, xlabel={ }, xticklabels=none, 
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{f1-timed};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name in \timedoracles{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
				}]  table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture}  
	\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={Timed DAG},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0, ymax= 1.1, width= 6cm, height=4.5cm,
			ylabel={TCG-F1}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
			legend entries={\textbf{gp},J-PCMCI,  R-PCMCI, 
   PCMCI+,  VARLiNGAM, DY-NOTEARS, CD-NOD}, legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, 
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{f1-timed};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name in \timedmethods{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
				}] table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture} 
 \begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={CPS},  
			 pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={CPS-F1}, xlabel={ }, xticklabels=none,  pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-f1}; 
			\def\file{\nonlinear};  
			\foreach \name in \cps{   
			\addplot+[area legend, boxplot = {%
				average = auto,%
				every average/.style={/tikz/mark=diamond*,/tikz/mar
    k size =2pt},%
			}, 
			]  table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture} 
		\begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={Partition  },  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={ARI}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
	 	%	legend entries={\textbf{gp}-kndag,\textbf{gp},R-PCMCI }, legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, , 
	 	pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-ari}; 
			\def\file{\nonlinear};  
			\foreach \name in \cps{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
					 }]  table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture}
			\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
		%	pretty ybar regime, 
			pretty boxplot regime, 
			title={Successes},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={Fract. successful runs}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
				legend entries={\textbf{gp}-kndag,\textbf{gp}, R-PCMCI
    },
    legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{valid};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name in \cps{   
				\addplot+[area legend]  table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture}
	\caption{ 	\label{fig:dag_search:boxes} \id }
\end{figure*}


==> figs/box/old/box_nlin_c5.tex <==
\def\oracles{gp-kncps, J-pcmci-kncps, % R-pcmci-kncps, R-pcmci-kncps,  
varLINGAM-kncps, dynotears-kncps, cdnod-kncps}
\def\timedoracles{gp-kncps, J-pcmci-kncps,  %R-pcmci-kncps, R-pcmci-kncps, 
varLINGAM-kncps, dynotears-kncps}
\def\cps{gp-kndag, gp} %, R-pcmci}
\def\methods{gp, J-pcmci, %R-pcmci,
pcmciplus, varLINGAM, dynotears, cdnod}
\def\timedmethods{gp, J-pcmci, %R-pcmci, 
pcmciplus, varLINGAM, dynotears}
\def\linear{expres/box/c_3_r_2_cps_3_n_3_t_200_d_1_i_2_ivs_50_f_lin_ns_unif.csv}
\def\nonlinear{expres/box/c_5_r_2_cps_4_n_5_t_200_d_1_i_2_ivs_50_f_exp_ns_gauss.csv} 
\def\id{\emph{nonlinear, gaussian noise, C5R2CPS4T200IV2}}
 %TODO show successes as a table next to CPS and next to DAG
\begin{figure*} [t] 
	\centering 
	\begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={CPS},  
			 pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={CPS-F1}, xlabel={ }, xticklabels=none,  pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-f1}; 
			\def\file{\nonlinear};  
			\foreach \name in \cps{   
			\addplot+[area legend, boxplot = {%
				average = auto,%
				every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},%
			}, 
			]  table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture} 
		\begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={Partition  },  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={ARI}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
	 	%	legend entries={\textbf{gp}-kndag,\textbf{gp},R-PCMCI }, legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, , 
	 	pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-ari}; 
			\def\file{\nonlinear};  
			\foreach \name in \cps{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
					 }]  table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture}
			\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
		%	pretty ybar regime, 
			pretty boxplot regime, 
			title={Successes},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={Fract. successful runs}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
				legend entries={\textbf{gp}-kndag,\textbf{gp}%R-PCMCI
    },
    legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{valid};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name in \cps{   
				\addplot+[area legend]  table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture}
	\begin{tikzpicture} 
	\begin{axis}[%legend image post style={mark=*}
		pretty boxplot regime, title={DAG, known CPS},  
		pretty enlargexlimits,  
		scatter src			= explicit symbolic,  
		cycle list name =prcl-box-time,
		pretty xlabelrot, 
		ymin = 0, ymax= 1.1,width= 6cm,height=4.5cm,
		ylabel={Dir. F1}, xlabel={ }, xticklabels=none, 
		pretty labelshift,
		] 
		% PARAMETERS
		\def\metric{f1};
		\def\var{C}; 
		\def\file{\nonlinear};  
		\foreach \name in \oracles{   
				\addplot+[ area legend, boxplot = {%
				average = auto,
				every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
			}]  table[y=\name_\metric] {\file};   
		}     
	\end{axis}
\end{tikzpicture}  
		\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={DAG},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0, ymax= 1.1, width= 6cm, height=4.5cm,
			ylabel={Dir. F1}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
			legend entries={\textbf{gp},J-PCMCI, %R-PCMCI,
   PCMCI+, VARLiNGAM, DY-NOTEARS, CD-NOD}, legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, 
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{f1};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name in \methods{   
				\addplot+[ area legend, boxplot = {%
				average = auto,
				every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
			}] table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture} 
	\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={Timed DAG, known CPS},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0, ymax= 1.1,width= 6cm,height=4.5cm,
			ylabel={TCG-F1}, xlabel={ }, xticklabels=none, 
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{f1-timed};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name in \timedoracles{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
				}]  table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture}  
	\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={Timed DAG},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0, ymax= 1.1, width= 6cm, height=4.5cm,
			ylabel={TCG-F1}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
			legend entries={\textbf{gp},J-PCMCI, % R-PCMCI, 
   PCMCI+,  VARLiNGAM, DY-NOTEARS, CD-NOD}, legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, 
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{f1-timed};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name in \timedmethods{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
				}] table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture}
	\caption{ 	\label{fig:dag_search:boxes} \id } 
\end{figure*}  

==> figs/box/old/box_nlin_unif.tex <==
\def\oracles{gp-kncps, J-pcmci-kncps, R-pcmci-kncps, R-pcmci-kncps,  
varLINGAM-kncps, dynotears-kncps, cdnod-kncps}
\def\timedoracles{gp-kncps, J-pcmci-kncps, R-pcmci-kncps, R-pcmci-kncps, 
varLINGAM-kncps, dynotears-kncps}
\def\cps{gp-kndag, gp, R-pcmci}
\def\methods{gp, J-pcmci, R-pcmci,
pcmciplus, varLINGAM, dynotears, cdnod}
\def\timedmethods{gp, J-pcmci, R-pcmci, 
pcmciplus, varLINGAM, dynotears} 
\def\nonlinear{expres/box/c_2_r_3_cps_2_n_5_t_200_d_1_i_0.5_ivs_50_f_exp_ns_unif_hi_False.csv}
\def\id{\emph{nonlinear, uniform noise, mechanism changes, N5C2R2CPS1T200IV0.5}}
 %TODO show successes as a table next to CPS and next to DAG
\begin{figure*} [t]
	\centering 
	\begin{tikzpicture} 
	\begin{axis}[%legend image post style={mark=*}
		pretty boxplot regime, title={DAG, known CPS},  
		pretty enlargexlimits,  
		scatter src			= explicit symbolic,  
		cycle list name =prcl-box-time,
		pretty xlabelrot, 
		ymin = 0, ymax= 1.1,width= 6cm,height=4.5cm,
		ylabel={Dir. F1}, xlabel={ }, xticklabels=none, 
		pretty labelshift,
		] 
		% PARAMETERS
		\def\metric{f1};
		\def\var{C}; 
		\def\file{\nonlinear};  
		\foreach \name in \oracles{   
				\addplot+[ area legend, boxplot = {%
				average = auto,
				every average/.style={/tikz/mark=diamond*,/tikz/mark size=2pt},% 
			}]  table[y=\name_\metric] {\file};   
		}     
	\end{axis}
\end{tikzpicture}  
		\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={DAG},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0, ymax= 1.1, width= 6cm, height=4.5cm,
			ylabel={Dir. F1}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
			legend entries={\textbf{gp},J-PCMCI, R-PCMCI,
   PCMCI+, VARLiNGAM, DY-NOTEARS, CD-NOD}, legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, 
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{f1};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name in \methods{   
				\addplot+[ area legend, boxplot = {%
				average = auto,
				every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
			}] table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture} 
	\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={Timed DAG, known CPS},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0, ymax= 1.1,width= 6cm,height=4.5cm,
			ylabel={TCG-F1}, xlabel={ }, xticklabels=none, 
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{f1-timed};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name in \timedoracles{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
				}]  table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture}  
	\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={Timed DAG},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0, ymax= 1.1, width= 6cm, height=4.5cm,
			ylabel={TCG-F1}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
			legend entries={\textbf{gp},J-PCMCI,  R-PCMCI, 
   PCMCI+,  VARLiNGAM, DY-NOTEARS, CD-NOD}, legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, 
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{f1-timed};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name in \timedmethods{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
				}] table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture} 
 \begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={CPS},  
			 pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={CPS-F1}, xlabel={ }, xticklabels=none,  pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-f1}; 
			\def\file{\nonlinear};  
			\foreach \name in \cps{   
			\addplot+[area legend, boxplot = {%
				average = auto,%
				every average/.style={/tikz/mark=diamond*,/tikz/mar
    k size =2pt},%
			}, 
			]  table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture} 
		\begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={Partition  },  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={ARI}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
	 	%	legend entries={\textbf{gp}-kndag,\textbf{gp},R-PCMCI }, legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, , 
	 	pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-ari}; 
			\def\file{\nonlinear};  
			\foreach \name in \cps{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
					 }]  table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture}
			\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
		%	pretty ybar regime, 
			pretty boxplot regime, 
			title={Successes},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={Fract. successful runs}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
				legend entries={\textbf{gp}-kndag,\textbf{gp}, R-PCMCI
    },
    legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{valid};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name in \cps{   
				\addplot+[area legend]  table[y=\name_\metric] {\file};   
			}     
		\end{axis}
	\end{tikzpicture}
	\caption{ 	\label{fig:dag_search:boxes} \id }
\end{figure*}


==> figs/box/oracle_dag_timed_cps.tex <==
\def\oracles{gp-kncps/\ns, J-pcmci-kncps/\ns, R-pcmci-kncps/\ns, pcmciplus/\ns,  
varLINGAM-kncps/\nsvlngkncps, dynotears-kncps/\ns, cdnod-kncps/\ns} 
\def\timedoracles{gp-kncps/\ns, J-pcmci-kncps/\ns, R-pcmci-kncps/\ns, R-pcmci-kncps/\ns, 
varLINGAM-kncps/\nsvlngkncps, dynotears-kncps/\ns}
\def\cps{gp-kndag/\ns, gp/\ns, R-pcmci/\nsrpcmci}
\def\cpsadjusted{gp-kndag/\nsgpkndagcps, gp/\nsgpcps, R-pcmci/\nsrpcmcicps}
\def\methods{gp/\ns, J-pcmci/\ns, R-pcmci/\nsrpcmci,
pcmciplus/\ns, varLINGAM/\ns, dynotears/\ns, cdnod/\ns}
\def\timedmethods{gp/\ns, J-pcmci/\ns, R-pcmci/\nsrpcmci, 
pcmciplus/\ns, varLINGAM/\ns, dynotears/\ns} 
 %TODO show successes as a table next to CPS and next to DAG
\begin{figure*} [t]
	\centering 
	\begin{tikzpicture} 
	\begin{axis}[%legend image post style={mark=*}
		pretty boxplot regime, title={DAG, known CPS},  
		pretty enlargexlimits,  
		scatter src			= explicit symbolic,  
		cycle list name =prcl-box-time,
		pretty xlabelrot, 
		ymin = 0, ymax= 1.1,width= 6cm,height=4.5cm,
		ylabel={Dir. F1}, xlabel={ }, xticklabels=none, 
		pretty labelshift,
		] 
		% PARAMETERS
		\def\metric{f1};
		\def\var{C}; 
		\def\file{\nonlinear};   
		\foreach \name/\succ in \oracles {   
				\addplot+[ area legend, boxplot = {%
				average = auto,
				every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
			}]  table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
		}     
	\end{axis}
\end{tikzpicture}  
		\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={DAG},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0, ymax= 1.1, width= 6cm, height=4.5cm,
			ylabel={Dir. F1}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
			legend entries={\textbf{gp},J-PCMCI, R-PCMCI,
   PCMCI+, VARLiNGAM, DY-NOTEARS, CD-NOD}, legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, 
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{f1};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \methods{   
				\addplot+[ area legend, boxplot = {%
				average = auto,
				every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
			}] table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}     
		\end{axis}
	\end{tikzpicture} 
	\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={Timed DAG, known CPS},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0, ymax= 1.1,width= 6cm,height=4.5cm,
			ylabel={TCG-F1}, xlabel={ }, xticklabels=none, 
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{f1-timed};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \timedoracles{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
				}]  table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}     
		\end{axis}
	\end{tikzpicture}  
	\begin{tikzpicture} 
		\begin{axis}[%legend image post style={mark=*}
			pretty boxplot regime, title={Timed DAG},  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,  
			cycle list name =prcl-box-time,
			pretty xlabelrot, 
			ymin = 0, ymax= 1.1, width= 6cm, height=4.5cm,
			ylabel={TCG-F1}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
			legend entries={\textbf{gp},J-PCMCI,  R-PCMCI, 
   PCMCI+,  VARLiNGAM, DY-NOTEARS, CD-NOD}, legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, 
			pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{f1-timed};
			\def\var{C}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \timedmethods{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
				}] table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}     
		\end{axis}
	\end{tikzpicture} 
 \begin{tabular}{ll}
\scriptsize{\textbf{method}} & \scriptsize{\textbf{successes}}       \\ \hline  
\scriptsize{ours}            & \scriptsize{\ns   /20}    \\
\scriptsize{ R-PCMCI }        & \scriptsize{\nsrpcmci /20 }\\
%\scriptsize{VARLiNGAM   }        & \scriptsize{\nsvlngkncps   /20  }  \\ 
\end{tabular} 
 \begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={CPS},  
			 pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={CPS-F1}, xlabel={ }, xticklabels=none,  pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-f1}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \cps{   
			\addplot+[area legend, boxplot = {%
				average = auto,%
				every average/.style={/tikz/mark=diamond*,/tikz/mar
    k size =2pt},%
			}, 
			]  table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}     
		\end{axis}
	\end{tikzpicture} 
 		\begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={Partition  },  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={ARI}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
	 	%	legend entries={\textbf{gp}-kndag,\textbf{gp},R-PCMCI }, legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, , 
	 	pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-ari}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \cps{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
					 }]  table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}     
		\end{axis}
	\end{tikzpicture}
 		\begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={Partition  },  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={NMI}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
	 	%	legend entries={\textbf{gp}-kndag,\textbf{gp},R-PCMCI }, legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, , 
	 	pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-nmi}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \cps{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
					 }]  table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}     
		\end{axis}
	\end{tikzpicture}
		\begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={Partition  },  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={ARI if perfect F1}, xlabel={ }, xticklabels=none, %symbolic x  coords={jpcmci, pcmci},
	 	%	legend entries={\textbf{gp}-kndag,\textbf{gp},R-PCMCI }, legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize}, , 
	 	pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-ari-adjusted}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \cpsadjusted{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
					 }]  table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}     
		\end{axis}
	\end{tikzpicture}
 		\begin{tikzpicture} 
		\begin{axis}[ 
			pretty boxplot regime, title={Partition  },  
			pretty enlargexlimits,  
			scatter src			= explicit symbolic,   
			pretty xlabelrot, ymin = 0, ymax= 1.1,
			ylabel={NMI if perfect F1}, xlabel={ }, xticklabels=none,
   				legend entries={\textbf{gp}-kndag,\textbf{gp}, R-PCMCI
    },
    legend columns=1, legend style=  {at = {(1.1, 1)}, anchor	= north west, font=\scriptsize},  
	 	pretty labelshift,
			] 
			% PARAMETERS
			\def\metric{cps-nmi-adjusted}; 
			\def\file{\nonlinear};  
			\foreach \name/\succ in \cpsadjusted{   
				\addplot+[ area legend, boxplot = {%
					average = auto,
					every average/.style={/tikz/mark=diamond*,/tikz/mark size =2pt},% 
					 }]  table[y=\name_\metric] {\file/successes_\succ/\name.csv};   
			}     
		\end{axis}
	\end{tikzpicture}   
\begin{tabular}{lll}
\scriptsize{\textbf{method}} & \scriptsize{\textbf{successful runs}}  & \scriptsize{\textbf{perfect CPS-F1}}       \\ \hline  
\scriptsize{ours}            & \scriptsize{\ns   /20}    & \scriptsize{\nsgpcps   /20}   \\
\scriptsize{ R-PCMCI }        & \scriptsize{\nsrpcmci /20 }   & \scriptsize{\nsrpcmcicps /20 }\\  
\end{tabular} 
	\caption{ 	\label{fig:dag_search:boxes} \id }
\end{figure*}


==> figs/cut_search/boxplots.tex <==
\def\file{regime_exp_data/res_linear.csv}
\pgfplotstableread[col sep=comma]{\file}\linear
\def\file{regime_exp_data/res_nonlinear.csv}
\pgfplotstableread[col sep=comma]{\file}\nlinear
% \def\method_names{\textbf{ours} (known regimes),\textbf{ours} (k.r.) \emph{(timed)},\textbf{ours} (5 bins),\textbf{ours} (5 bins) \emph{(timed)},JPCMCI+,JPCMCI+\emph{(timed)},VarLiNGAM-$c$,VarLiNGAM-$C$}

% sorry for the ugly figs, i don't want to loose time to do nice figs that may be deleted later

\begin{figure*}[t]
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        pretty boxplot,
        ylabel={Metric},
        xtick={1.5, 3.5},
        xticklabels={Precision, Recall},
        legend entries={linear, non-linear}, 
        legend columns=1
        ]
        
        \addplot+[fill=airforceblue, area legend] table[y=precision] {\linear}; 
        \addplot+[fill=amber, area legend] table[y=precision] {\nlinear}; 
        \addplot+[fill=airforceblue, area legend] table[y=recall] {\linear}; 
        \addplot+[fill=amber, area legend] table[y=recall] {\nlinear}; 
     
    \end{axis}
    \end{tikzpicture}	
    \caption{ 
    \label{fig:cut_search:changepointsboxplot} Change point identification performance.}
\end{figure*}

\begin{figure*}[t]
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        pretty boxplot,
        ylabel={Metric},
        xtick={1.5, 3.5},
        xticklabels={AMI, ARI},
        legend entries={linear, non-linear}, 
        legend columns=1
        ]
        
        \addplot+[fill=airforceblue, area legend] table[y=ami] {\linear}; 
        \addplot+[fill=amber, area legend] table[y=ami] {\nlinear}; 
        \addplot+[fill=airforceblue, area legend] table[y=ari] {\linear}; 
        \addplot+[fill=amber, area legend] table[y=ari] {\nlinear};  
     
    \end{axis}
    \end{tikzpicture}		
    \caption{ 
    \label{fig:cut_search:regimeboxplot} Regime partition performance.}
\end{figure*}


==> figs/illustrations/consistency.tex <==
\begin{figure}[b]
\begin{tikzpicture}[font=\small,thick]
\tikzset{question_node/.style={draw,
    rectangle,
    rounded corners = 2pt,
    minimum width=3cm,
    minimum height=1cm}}
\tikzset{task_node/.style={ draw,
    rectangle, 
    rounded corners = 2pt,
    minimum width=2.7cm,
    minimum height=0.5cm,
    inner sep=1}}
\tikzset{case_node/.style={ draw,
    rectangle, 
    rounded corners = 2pt,
    minimum width=2.5cm,
    minimum height=0.5cm,
    inner sep=1}}
\tikzset{proof_node/.style={    
    minimum width=2.5cm,
    inner sep=0.2}}
    
% Start 
\node[question_node] (block1) {Cutpoints $\cps$ known};
   
\node[question_node, below left =of block1] (block2) { Partitions $\R, \C$ known};

% causal dag
\node[ task_node,
    below left=of block2, fill=white ] (block5) {\textbf{Causal DAG Discovery}};
    
% markov equivalence
\node[question_node,
    below=of block5] (block6) { Markov Equivalence  $\Gh \sim \Gs$ };
\node[  case_node,
    below =0.5cm  of block6 ] (block6a) {Case $\Gh \supsetneq \Gs$  };
\node[  proof_node, 
    below =0.5cm of block6a] (block6aa) { Causal Markov, Faithfulness };

\node[ case_node, 
    below=0.5cmof block6aa ] (block6c) { Case $\Gh \subsetneq \Gs$  };
\node[  proof_node, 
    below=0.5cm of block6c ] (block6cc) {  $D_{\text{KL}}$ terms  };
     
    
% causal directions 
\node[ question_node, 
    %below =of block6cc
    right = of block6
    ] (block7) {Causal Directions $\Gh = \Gs$ };
 
\node[  case_node, 
    below= of block7,     minimum width=3cm ] (block7a) {Edge  $\iX i \to \iX j$};
\node[  proof_node,
    below=0.5cm of block7a ] (block7aa) {Independent Change $Z_{(i)} \indep Z_{(j)} $};
\node[   
    below=0.5cm of block7aa ] (block7aaa) { };

    
% causal mechanisms
\node[ task_node,
    below right= of block2 ] (block4) {\textbf{Change Identification}};
\node[  case_node,
    below =0.5cm of block4 ] (block4a) { Case $\Rh \undernegsuccurlyeq \Rs$ };
\node[  proof_node, 
    below =0.5cm of block4a] (block4aa) { Shift Faithfulness };

\node[ case_node, 
    below=0.5cm   of block4aa ] (block4b) { Case $\Rh \undernegpreccurlyeq \Rs$  };
\node[  proof_node, 
    below=0.5cm of block4b ] (block4bb) {  $D_{\text{KL}}$ terms  };

% cutpoints 
\node[task_node, right = of block4] (block3) { \textbf{Cutpoint Detection} };
  
\node[  case_node,
    below =0.5cm of block3 ] (block3a) { Case $\Ph \undernegsuccurlyeq  \Ps$ };
\node[  proof_node, 
    below =0.5cm of block3a] (block3aa) { Shift Faithfulness 
    };

\node[ case_node, 
    below=0.5cm   of block3aa ] (block3b) { Case $\Ph \undernegpreccurlyeq \Ps$  };
    
\node[  proof_node, 
    below=0.5cm of block3b ] (block3bb) { $D_{\text{KL}}$ terms  };

 
% Return block
\node[draw,
    rounded rectangle,
    below=7cm of block4,
    minimum width=2.5cm,
    minimum height=1cm,] (block11) { $\big( \Gh, \Ph, \Rh , \Ch \big) = \big( \Gs, \Ps, \Rs , \Cs \big)  $};

\node[coordinate,below=6.35cm of block4] (block12) {};


% Arrows
%\draw[-latex] (block1) edge (block2)
%    (block2) edge (block3)
%    (block3) edge (block4);

\draw[-latex] (block1) -| (block2)
    node[pos=0.25,fill=white,inner sep=0]{Yes};
    
\draw[-latex] (block1) -| (block3)
    node[pos=0.25,fill=white,inner sep=0]{No};

\draw[-latex] %(block2) edge node[pos=0.4,fill=white,inner sep=2pt]{No}(block4)
    (block2) -| (block4)
        node[pos=0.25,fill=white,inner sep=0]{No};
 \draw[-latex]    (block2) -| (block5)
        node[pos=0.25,fill=white,inner sep=0]{Yes};
        
%\draw[-latex] (block6) edge node[pos=0.4,fill=white,inner sep=2pt]{No}(block9)
%    (block6) -| (block10)
%        node[pos=0.25,fill=white,inner sep=0]{Yes};

\draw (block6) |- (block5);
\draw (block7) |- (block5);
\draw (block6cc) |- (block12);
\draw (block7aa) |- (block12);
\draw (block3bb) |- (block12);
\draw (block4bb) |- (block12);
%\draw (block5) |- (block7|-block12);
%\draw (block10) |- (block3a|-block3bb); 
\draw[-latex] (block12) -- (block11);

\end{tikzpicture}
\caption{\emph{Consistency.} Depiction of the cases in the consistency proof.}
\end{figure}

==> figs/illustrations/mixture_model.tex <==
\tikzset{ 
	plate/.style={draw=black, thick,  rounded corners,
		inner xsep=1em,
		inner ysep=1.2em},
	latent_plate/.style={draw=black, densely dotted, rounded corners,
		inner xsep=1em,
		inner ysep=1em}
  }
\begin{figure}[b]
	\begin{center}
		\tikz{ 
			\tikzstyle{obs}=[shape=circle,thick,draw,fill=black!20]
			\tikzstyle{latent}=[shape=rectangle, rounded corners,thick,draw]
			\tikzstyle{latent_param}=[shape=rectangle, rounded corners,thick, %draw, black!70
   ]
			% nodes
			\node[obs] (y) {$X_j$}; 
			\node[latent, scale=1, above=of y] (z)  {$Z_j$} ;   
			\node[below=1.5cm of z] (z2) {$\quad\quad\quad$}; 
			\node[left=of z] (x2) {}; 
			\node[obs, left=of y, scale=1] (x) {$X_i$}; 
			\node[latent, circle, above  =of x] (n)  {$N_j$}
		%	\node[latent, above=of z] (c) {$\C \times \R$};
			\node[latent_param, right=1.2cm of y] (mu) {$\boldsymbol{\theta}_j $}; 
			\node[latent_param, right=1.2cm of z] (pi) {$\boldsymbol{\pi}_j$};
		%	\node[ right=of c] (pi2) { };
   %todo use absolute coordinates
			\node[below right=1.6cm and 1.1cm of z] (mu2) {};  
			% edges
			\path [->,draw,thick] 
			(x) edge (y) 
			(n) edge (y) 
                (z) edge (y);
			\path [->,draw,dotted,thick] 
			%(c) edge (z)
			(pi) edge (z)
			(mu) edge (y) ;
		\node[above = .4cm of z] (dt)
		{\scriptsize{$ \dsz  \times  \tsz $}}; 
	%	\node[above = .4cm of pi] (cr)
	%	{\scriptsize{$\quad \csz \times  \rsz $}};
		\node[plate, fit=(x) (dt)] {};
	%	\node[latent_plate, fit=(pi) (cr)] {}; 
	 }
		\caption{\emph{Augmented causal model}. We illustrate our causal model in plate notation. Each variable is associated with  causal   parameters $\theta$, an exogenous noise variable $N$, and a regime-context confounder $Z$, here shown for  $X_j$. Solid edges denote causal edges,  white nodes unobserved variables, gray ones observed variables, and circles continous-valued variables, squares discrete-valued variables. }
		\label{fig:illustrations:mixture_model}
	\end{center}
\end{figure}

==> figs/realworld/fluxnet_tsne.tex <==
\pgfplotsset{ 
    colormap={ourmap}{
        rgb255=(251,191,36) 
        rgb255=(22,161,74) 
        rgb255=(3,105,161) 
        rgb255=(131,24,76)
    },
} 
\pgfplotsset{ colormap={ourmap}{
rgb255=(251,191,36) rgb255=(22,161,74) rgb255=(3,105,161) rgb255=(131,24,76)}%
}%    %rgb255=(12,74,110), 
\pgfplotsset{colormap/ourmap} 
\begin{figure*}[t] 
    \begin{subfigure}[c]{0.22\textwidth}
     \begin{tikzpicture}[->,>=stealth, node distance=1cm, every node/.style={draw, thick, font=\small}] 
		\foreach[count=\i,evaluate=\i as \angle using (\i)*360/6] \text in {%
			VPD,LE,H,NEE,R,T
		}
		\node[] (n\i) [dag_node, fill=slate200] at (\angle:1.1) {}; %{\scriptsize \text};  
  %Edges
		\draw [dag_edge] (n5) edge (n3); 
		\draw [dag_edge] (n2) edge (n5); 
		\draw [dag_edge] (n5) edge (n4); 
		\draw [dag_edge] (n5) edge (n1); 
		\draw [dag_edge] (n3) edge (n2); 
		\draw [dag_edge] (n1) edge (n2);   
		\draw [dag_edge] (n1) edge (n6);  

every node/.style={thick, font=\small}] 
		\foreach[count=\i,evaluate=\i as \angle using (\i)*360/6] \text in {%
			VPD,LE,H,NEE,R,T
		}
		\node[] (n\i) [draw=none] at (\angle:1.55) {\emph{\text } };  

        \end{tikzpicture}
        \caption{Summary DAG.}
    \end{subfigure} 
 \begin{subfigure}[c]{.55\textwidth} 
 \centering
\begin{minipage}{.5\textwidth} 
\begin{tikzpicture}
    \begin{axis}[pretty heated horizontal, height=4.25cm, width=4.25cm,
        colorbar,
        mesh/interior colormap name=hot, 
        %colormap name=ourmap,
        colormap={ourmap}{rgb255=(251,191,36) rgb255=(22,161,74) rgb255=(3,105,161) rgb255=(131,24,76)},
        scatter/use mapped color={draw=mapped color!80, fill=mapped color!80},
        colorbar sampled,
        colorbar style={samples=6,
       xtick={0,  1},
            % vertical version: width=.25cm, height=1.5cm, xshift=-0.1cm,    yshift=-1.4cm,          
            % horizontal version:
            height=0.2cm, width=1.4cm, xshift=.2cm,    yshift=4.5cm, %vertical           
            ticklabel style={
                /pgf/number format/fixed,    % To ensure fixed-point notation
                /pgf/number format/precision=2, % Number of decimals
                font=\scriptsize,        
			xlabel   ={Edge strengths $\delta E$
   }, 
            }, 
            xtick={0,1},xticklabels={0,1},
                xticklabel style={
                font=\tiny,  text width=.5em,
            align=right,
            /pgf/number format/.cd,
                fixed,
                fixed zerofill
        }
        }, 
        mark size=1pt,
        xlabel={T-SNE $x_1$}, 
        ylabel={T-SNE $x_2$}, xmax=120, xmin =-120, ymax=100, ymin=-100, %xticklabels= {-50,,,,,0,,,,, 50},%
        xticklabels=  {-100,,,,0,,,,100}, %{-120,,,,,,0,,,,,, 120},
        yticklabels= {-100,,,,0,,,,100}, 
       xtick= {-100, -75, -50, -25, 0, 25, 50, 75, 100}, ytick= {-100, -75, -50, -25, 0, 25, 50, 75, 100}, %{-120, -100, -80, -60, -40, -20, 0, 20, 40, 60, 80, 100, 120}, 
        pretty labelshift
    ] 
    \addplot+[
        scatter,
        point meta=explicit,  % Use explicit color values
    ] table[meta=col] {expres/realworld/fluxnet_tsne_strength_3_sub.csv}; 
    \end{axis} 
\end{tikzpicture}  
\end{minipage}
\begin{minipage}{.45\textwidth} 
\begin{tikzpicture}[->,>=stealth]
    \begin{axis}[pretty line marks, height=4.25cm, width=4.25cm,
    axis y line=none,
        mark size=1.2pt,
        xlabel={}, 
        ylabel={}, xmax=120, xmin =-120,  
        xticklabels=  {},  
        yticklabels= {},
       xtick= {}, ytick= {}, tick label style={color=white},
        pretty labelshift
    ] 
    \addplot+[slate200!70] table[meta=col] {expres/realworld/fluxnet_tsne_strength_3_sub.csv}; 
    %fluxnet_tsne_strength_yearavg.csv}; 
    \end{axis}
    % Top-left mini graph: sparse
    \begin{scope}[shift={(.8cm, 2.3cm)}, scale=0.4]
        \foreach[count=\i,evaluate=\i as \angle using (\i)*360/6] \text in {%
            VPD,LE,H,NEE,R,T
        }
       \node[circle, draw, fill=black, minimum size=0.1cm, inner sep=0] (n\i) at (\angle:1) {};  
       %TYPE 3,  NEE and LE strongly connected 
		\draw [w4] (n2) edge (n5);    %not strongest
		\draw [w2, strongest] (n5) edge (n4);   
		\draw [w3] (n5) edge (n3); %not strongest
		\draw [w1] (n5) edge (n1);    %not strongest   
		\draw [w3, strongest] (n1) edge (n2);   
		\draw [w1] (n1) edge (n6);   %not strongest 
    \end{scope}
    % Top-right mini graph: sparse
    \begin{scope}[shift={(2.3cm,2.3cm)}, scale=0.4]
        \foreach[count=\i,evaluate=\i as \angle using (\i)*360/6] \text in {%
            VPD,LE,H,NEE,R,T
        }
       \node[circle, draw, fill=black, minimum size=0.1cm, inner sep=0] (n\i) at (\angle:1) {};   
         %TYPE 4,  all strongly connected
    \draw [w4, strongest] (n5) edge (n3); 
    \draw [w4, strongest] (n2) edge (n5); 
    \draw [w1] (n5) edge (n4); %not strongest
    \draw [w3, strongest] (n5) edge (n1); 
    \draw [w1, strongest] (n3) edge (n2); 
    \draw [w1] (n1) edge (n2);   %not strongest   
    \draw [w2] (n1) edge (n6);  %not strongest  
    \end{scope}

    % Bottom-left mini graph: weakly connected
    \begin{scope}[shift={(.8cm, .8cm)}, scale=0.4]
        \foreach[count=\i,evaluate=\i as \angle using (\i)*360/6] \text in {%
            VPD,LE,H,NEE,R,T
        }
        \node[circle, draw, fill=black, minimum size=0.1cm, inner sep=0] (n\i) at (\angle:1) {};
       %TYPE 0, SPARSE GRAPH
		\draw [w1] (n1) edge (n6);  
		\draw [w1] (n5) edge (n1);  
		\draw [w1] (n3) edge (n2);   
    \end{scope} 
 % Bottom-right mini graph: T
    \begin{scope}[shift={(2.2cm, .8cm)}, scale=0.4] % Scale applied
        \foreach[count=\i,evaluate=\i as \angle using (\i)*360/6] \text in {%
            VPD,LE,H,NEE,R,T
        }
        \node[circle, draw, fill=black, minimum size=0.1cm, inner sep=0] (n\i) at (\angle:1) {}; 
        %TYPE 2, T strongly, others sparsely connected
		\draw [w4] (n5) edge (n3);   %not strongest
		\draw [w3, strongest] (n1) edge (n6);   
		\draw [w2] (n5) edge (n1);   %not strongest 
    	\draw [w1] (n2) edge (n5);   %not strongest 
    \end{scope}
\end{tikzpicture}
\end{minipage}
        \caption{Edge Strengths for each Location and Month.} 
\end{subfigure} 
    % Time Series Plots
   \begin{comment}
    \begin{subfigure}[c]{0.2\textwidth} 
        \begin{tikzpicture}
        \begin{axis}[
            scale only axis,
            width=2.5cm,
            height=3cm,
            axis x line=none,  
            axis y line=none,  
            xtick=\empty,
            ytick=\empty,
            xmin=0 
        ] 
        \node[draw=none] at (axis cs:\poslabelts,0) {$X_{(1)}$}; 
        \addplot[\colorregimeone, mark=none, unbounded coords=jump, x filter/.expression={x>33 && x<66 ? nan : x+\xshiftts}] table [col sep=comma, x=t, y=a] {figs/illustrations/timeseries1.csv};
        
        \addplot[\colorregimetwo, mark=none, unbounded coords=jump, x filter/.expression={x<33 || x>66 ? nan : x+\xshiftts}] table [col sep=comma, x=t, y=a] {figs/illustrations/timeseries1.csv};
        
        \addplot[black, mark=none, y filter/.expression={y-\yshiftts}, x filter/.expression={x+\xshiftts}]  table [col sep=comma, x=t, y=b] {figs/illustrations/timeseries1.csv};
        \node[draw=none] at (axis cs:\poslabelts,-\yshiftts) {$X_{(2)}$}; 
 
        \node[draw=none] at (axis cs:\poslabelts,-2*\yshiftts) {$X_{(3)}$};
        \addplot[\colorcontextone, mark=none, y filter/.expression={y-(\yshiftts*2)}, x filter/.expression={x+\xshiftts}] table [col sep=comma, x=t, y=c] {figs/illustrations/timeseries1.csv};

        \end{comment}
       % \node[draw=none] at (axis cs:\poscontextts,-\yshiftts) {$C_1$}; 

        \begin{comment}
        \node[draw=none] at (axis cs:\poslabelts,-4*\yshiftts) {$X_{(1)}$}; 
        \addplot[\colorregimeone, mark=none, y filter/.expression={y-4*\yshiftts}, unbounded coords=jump, x filter/.expression={x>33 && x<66 ? nan : x+\xshiftts}] table [col sep=comma, x=t, y=a] {figs/illustrations/timeseries2.csv};


        \addplot[\colorregimetwo, mark=none, y filter/.expression={y-4*\yshiftts}, unbounded coords=jump, x filter/.expression={x<33 || x>66 ? nan : x+\xshiftts}] table [col sep=comma, x=t, y=a] {figs/illustrations/timeseries2.csv};
               
        \addplot[black, mark=none, y filter/.expression={y-5*\yshiftts}, x filter/.expression={x+\xshiftts}]  table [col sep=comma, x=t, y=b] {figs/illustrations/timeseries2.csv};
        \node[draw=none] at (axis cs:\poslabelts,-5*\yshiftts) {$X_{(2)}$};
 
        \node[draw=none] at (axis cs:\poslabelts,-6*\yshiftts) {$X_{(3)}$};
        \addplot[\colorcontexttwo, mark=none, y filter/.expression={y-(\yshiftts*6)}, x filter/.expression={x+\xshiftts}] table [col sep=comma, x=t, y=c] {figs/illustrations/timeseries2.csv};

        \node[draw=none] at (axis cs:\poscontextts,-\yshiftts*5) {$C_2$}; 

        \def\ytimeline{-7.1*\yshiftts}
        \addplot[draw=none] coordinates{(\xshiftts,\ytimeline) (\xshiftts+100,\ytimeline-3)};
        \draw[->] (axis cs:\xshiftts,\ytimeline) -- (axis cs:\xshiftts+100,\ytimeline);
        \addplot[mark=|] coordinates{(\xshiftts+33,\ytimeline) (\xshiftts+66,\ytimeline)};
        \draw[->, thin] (axis cs:\xshiftts,\ytimeline) -- (axis cs:\xshiftts+100,\ytimeline);
        \node[draw=none] at (axis cs:\xshiftts+105,\ytimeline) {$t$};
        \draw[thin, decorate,decoration={brace,amplitude=6pt,mirror}] (axis cs:\xshiftts, \ytimeline) -- (axis cs:\xshiftts+33, \ytimeline) node [black,below=5pt,midway]  {$R_1$};
        \draw[thin, decorate,decoration={brace,amplitude=6pt,mirror}] (axis cs:\xshiftts+33, \ytimeline) -- (axis cs:\xshiftts+66, \ytimeline) node [black,below=5pt,midway] {$R_2$};
        \draw[thin, decorate,decoration={brace,amplitude=6pt,mirror}] (axis cs:\xshiftts+66, \ytimeline) -- (axis cs:\xshiftts+100, \ytimeline) node [black,below=5pt,midway] {$R_1$};
        
        \end{comment}
        \end{axis}
        \end{tikzpicture}
 
        \caption{Regime Partitioning.} 
\end{subfigure}
\caption{ \label{fig:flux} \emph{Biosphere-Atmosphere Interactions.} For the FLUXNET database with 64 locations $\D$ over multiple years $\T$, we show the summary DAG (left) that we discover with \ourmethodns.  The T-SNE embedding  (middle) visualizes the causal edge strengths, where each sample $(x_1, x_2)$ corresponds to a fixed location $d_i$, month $m_i$, and year $y_i$. We recover different regions that correspond to distinct underlying meteorological conditions (strongly connected vs. weakly connected: high vs. low precipitation; strong connectivity towards NEE and LE vs. towards T: medium vs. high radiation). Finally, regime partitioning (right) reveals abnormal trends, such as a causal mechanism shift in 2003 for the selected location $d_i:$ DeThai due to an observable difference in precipitation.  }
\end{figure*}


==> figs/realworld/river_cps_search.tex <==
\def\yrsRzeroDeHai{2000,2001,2002,2004,2005,2006,2007,2008} 
\def\yrsRoneDeHai{2003} 
\def\yrsRtwoDeHai{2009,2010,2011}
%detha, itro1
        %[(0, 46, 0.0), (46, 31, 1.0), (77, 34, 2.0), (111, 79, 1.0), (190, 30, 3.0), (220, 35, 1.0), (255, 46, 2.0), (301, 31, 4.0), (332, 33, 5.0)]
      %_[(0, 114, 0.0), (114, 30, 1.0), (144, 50, 2.0), (194, 66, 3.0), (260, 105, 4.0)]
\begin{figure}[t] 
  %  \begin{subfigure}[c]{0.25\textwidth} 
        \begin{tikzpicture}
        \begin{axis}[
            scale only axis,
            width=8cm,
            height=3cm,
            axis x line=none,  
            axis y line=none,  
            xtick=\empty,
            ytick=\empty,
            xmin=0,
            legend entries={}, % {runoff \emph{Q}},
            legend image post style={xscale=.4, yscale=1}, 
            legend style={font=\tiny},
        ]  
        \addplot[\colorcontextone, mark=none,  unbounded coords=jump, % x filter/.expression={x>45 && x<77 ? nan : x},
        line width=1.5pt,
        ] table [x=t, y=Qobs, col sep=comma] %5_6935145_2010.csv
        {expres/river_texdata/6_6604220_2010.csv}; 
      %_[(0, 114, 0.0), (114, 30, 1.0), (144, 50, 2.0), (194, 66, 3.0), (260, 105, 4.0)]
        \end{axis}
        \end{tikzpicture}
     %   \caption{Changepoints $\cps$ and regimes $\R$.}
      %  \end{subfigure}
    \caption{\emph{Changepoints of the Interaction between Precipitation and Runoff.} We show the regime changepoints $\cps$ and partition \emph{Q} that we discover for  $P \to \emph{Q}$ with \ourmethod for selected catchments $d$ in the river discharge data.}
    \label{fig:river_regimes}
\end{figure}

==> figs/test/line_nlin.tex <==
\def\methods{gp, J-pcmci}
\begin{figure*} [t]
	\centering
	\begin{tikzpicture}
	\begin{axis}[
        pretty line regime,
	ylabel={F1}, xlabel={Variables $N$}
	] 
	\def\metric{f1};
	\def\var{N};
	\def\file{expres/C1_D1_R2_T200_Fnlin_vary_N.csv};
	\foreach \name in \methods{   
			\addplot table[x = \var, y = \name_\metric] {\file};   
			\addplot[forget plot,name path=lower, fill=none, draw=none, smooth] 
			table [ x=\var, y expr=\thisrow{\name_\metric} - \thisrow{\name_\metric_var} ]{\file};
			\addplot[forget plot,name path=upper, fill=none, draw=none, smooth] 
			table [ x=\var, y expr=\thisrow{\name_\metric} + \thisrow{\name_\metric_var} ]{\file};
			\addplot fill between[of=lower and upper];
	}     
	\end{axis}
	\end{tikzpicture}		\begin{tikzpicture}
	\begin{axis}[
        pretty line regime,
	ylabel={F1}, xlabel={Contexts $\C$}, xmax  =20
	] 
	\def\metric{f1};
	\def\var{C};
	\def\file{expres/D1_R2_T200_N2_Fnlin_vary_C.csv};
	\foreach \name in \methods{   
			\addplot table[x = \var, y = \name_\metric] {\file};   
			\addplot[forget plot,name path=lower, fill=none, draw=none, smooth] 
			table [ x=\var, y expr=\thisrow{\name_\metric} - \thisrow{\name_\metric_var} ]{\file};
			\addplot[forget plot,name path=upper, fill=none, draw=none, smooth] 
			table [ x=\var, y expr=\thisrow{\name_\metric} + \thisrow{\name_\metric_var} ]{\file};
			\addplot fill between[of=lower and upper];
	}     
	\end{axis} 
	\end{tikzpicture}   
	\caption{ 	\label{fig:dag_search:bar_lin}   The effect of increasing the number of nodes (left) or contexts (right). The base settings are nonlinear, $N=2$ nodes,  $|C|=1$ contexts and datasets with $n=200$ time points and split into $R=2$ regimes. \notes{todo: change to larger $n$, $C$ and $N$ as otherwise JPCMCI not working yet; also show with increasing $R$ that methods assuming stationarity get worse then.}}
\end{figure*}

==> figs/test/testing.tex <==
\def\methods{gp, J-pcmci}
\def\file{expres/lin_D1_R2_N2_Flin_vary_C.csv}
\def\var{C}

\def\method_names{\textbf{ours} (known regimes),\textbf{ours} (k.r.) \emph{(timed)},\textbf{ours} (5 bins),\textbf{ours} (5 bins) \emph{(timed)},JPCMCI+,JPCMCI+\emph{(timed)},VarLiNGAM-$c$,VarLiNGAM-$C$}

\begin{figure*}[t]
	\centering
	\begin{tikzpicture}
	\begin{axis}[
        pretty ybar regime,
	ylabel={F1}
	] 
	\def\metric{f1};
	\foreach \name in \methods{   
		\addplot table[x =\var, y=\name_\metric] {\file}; 
	}     
	\end{axis}
	\end{tikzpicture}		
        \begin{tikzpicture}
	\begin{axis}[ 
        pretty ybar regime,
	ylabel={SHD}
	] 
	\def\metric{shd};  
	\foreach \name in \methods{   
		\addplot table[x =\var, y=\name_\metric] {\file}; 
	}     
	\end{axis}
	\end{tikzpicture}
		\begin{tikzpicture} 
	\begin{axis}[
        pretty ybar regime,
	ylabel={TPR}
	] 
	\def\metric{tpr};  
	\foreach \name in \methods{   
		\addplot table[x =\var, y=\name_\metric] {\file}; 
	}     
	\end{axis}
	\end{tikzpicture}
	\begin{tikzpicture}
	\begin{axis}[
        pretty ybar regime, 
	legend entries={\textbf{ours} (known regimes),\textbf{ours} (k.r.) \emph{(timed)},\textbf{ours} (5 bins),\textbf{ours} (5 bins) \emph{(timed)},JPCMCI+,JPCMCI+\emph{(timed)},VarLiNGAM-$c$,VarLiNGAM-$C$}, legend columns=1,
			] 
			\def\metric{fpr}; 
			\foreach \name in \methods{   
				\addplot table[x =\var, y=\name_\metric] {\file}; 
			}     
	\end{axis}
	\end{tikzpicture}   
	\caption{ 
	\label{fig:dag_search:bar_lin}  Caption.}
\end{figure*}

==> rebuttal_draft.tex <==
\onecolumn
Limit: 2500 characters per reviewer (less than the number of characters used by reviewer 1 for its questions).

\section{Reviewer 1}
Thank you for your detailed comments. Due to the character limit we can only address some of your questions.
\paragraph{Notation} Fair points. We will reconsider and clarify the notation. (Q4) $\mathcal C(d) = k$ is a deterministic function that assigns dataset $d$ to context $C_k$. (Q5) $X^d_t$ in Asm. 3 refers to one observation of node $i$ at time $t$ in $d$.
\paragraph{Non-i.i.d.-ness} (Q15) While we can address non-i.i.d.-ness due to function changes, our theory assumes the samples generated by the sliding window approach to be i.i.d. Specifically, we assume consistent GP regression estimation (Def. 10) of all functions $f^{r,k}_{i}$. If this does not hold and parent sets are incorrect, spurious regime changes could be detected but no true changepoints will be missed, i.e. regimes remain pure. Our experiments suggest parent sets are mostly correct in practice. An auto-regressive approach is common, but an analysis of the effect of non-i.i.d.-ness on consistency seems to be missing from the score-based literature for time series. We will include this as a limitation. 
\paragraph{Complexity} (Q8) The complexity of our method is $\mathcal O(n^2 + |V|^3n^3 +(n_{R}^2+n_{C}^2)n_{TD}^3)$ with $n_{TD}=n|D|, n_C=|D|, n_R=\left \lfloor{n/d_{min}}\right \rfloor$.
\paragraph{Convergence} (Q18) Yes. We only accept changes to the model that improve its score, which in turn is lower bounded by 0. Under any $G$, changes at true changepoints lead to changes in $P(X \mid pa(G))$ due to faithfulness. This suggests that changepoint search discovers a (super)set of the true changepoints even under incorrect $G$ (initially, the empty graph) and then converges quickly.
\paragraph{Experiments} (Q17) In short, we follow the data generation of JPCMCI (github.com/jakobrunge/tigramite) with the modification that we also sample regimes in which for certain $i$ we replace $f^{k,r}_{(i)}$. (Q19) We apply the methods (except: ours, JPCMCI) to each $d$ in turn; in each $d$, we apply the methods (except: ours, RPCMCI) either to each window (known changepoints), or all samples (unknown changepoints). We aggregate results with majority voting. 
(Q20) We chose $n=200$ to demonstrate that our method is sample-efficient, but agree that showing the effect of sample size will be insightful. To illustrate, with $n=500$ our method ($0.78\pm0.13 F1-G$) performs well compared to JPCMCI ($0.4\pm0.31$), PCMCI+ ($0.6\pm0.19$). We also ran PCMCI+ without voting, on all $d$ combined with $n=1000$ ($0.55\pm0.13$).

% Thank you for your detailed comments. Due to the character limit we can only address some of your questions.

% **Notation** Fair points. We will reconsider and clarify the notation. (Q4) $\mathcal C(d) = k$ is a deterministic function that assigns dataset $d$ to context $C_k$. (Q5) $X^d_t$ in Asm. 3 refers to one observation of node $i$ at time $t$ in $d$.

% **Non-i.i.d.-ness** (Q15) While we can address non-i.i.d.-ness due to function changes, our theory assumes the samples generated by the sliding window approach to be i.i.d. Specifically, we assume consistent GP regression estimation (Def. 10) of all functions $f^{r,k}_{i}$. If this does not hold and parent sets are incorrect, spurious regime changes could be detected but no true changepoints will be missed, i.e. regimes remain pure. Our experiments suggest parent sets are mostly correct in practice. An auto-regressive approach is common, but an analysis of the effect of non-i.i.d.-ness on consistency seems to be missing from the score-based literature for time series. We will include this as a limitation. 

% **Complexity** (Q8) The complexity of our method is $\mathcal O(n^2 + |V|^3n^3 +({n_{R}}^2+{n_{C}}^2){n_{TD}}^3)$ with $n_{TD}=n|D|, n_C=|D|, n_R=\left \lfloor{n/d_{min}}\right \rfloor$.

% **Convergence** (Q18) Yes. We only accept changes to the model that improve its score, which in turn is lower bounded by 0. Under any $G$, changes at true changepoints lead to changes in $P(X \mid pa(G))$ due to faithfulness. This suggests that changepoint search discovers a (super)set of the true changepoints even under incorrect $G$ (initially, the empty graph) and then converges quickly.

% **Experiments** (Q17) In short, we follow the data generation of JPCMCI (github.com/jakobrunge/tigramite) with the modification that we also sample regimes in which for certain $i$ we replace $f^{k,r}_{(i)}$. (Q19) We apply the methods (except: ours, JPCMCI) to each $d$ in turn; in each $d$, we apply the methods (except: ours, RPCMCI) either to each window (known changepoints), or all samples (unknown changepoints). We aggregate results with majority voting. 
% (Q20) We chose $n=200$ to demonstrate that our method is sample-efficient, but agree that showing the effect of sample size will be insightful. To illustrate, with $n=500$ our method ($0.78\pm0.13$ F1-G) performs well compared to JPCMCI ($0.4\pm0.31$), PCMCI+ ($0.6\pm0.19$). We also ran PCMCI+ without voting, on all $d$ combined with $n=1000$ ($0.55\pm0.13$).


\section{Reviewer 2} 
Thank you for your detailed comments. 
\paragraph{Problem setting} Yes, our approach allows multiple variables to change at the same time. We set a changepoint $l \in \mathcal L$ whenever \emph{at least} one node $i$ changes at $l$, but the output of our method will show which variable sets change at which locations. We will clarify this in the problem-setting section.
\paragraph{Complexity} We inherit the complexities of the chosen components, namely PELT in $\mathcal O(n^2)$, where $n=|\mathcal T|$; Causal Discovery in $\mathcal O({n_V}^3)$ (Mian et al. 2021) for $n_V$ nodes, together with GP regression in $\mathcal O({n_{s}}^3)$ for $n_{s}$ samples;
and partitioning in $O((n_{R}^2+n_{C}^2)n_{TD}^3)$ as the kernel test is applied to pairs of regimes and contexts, where $n_{R},n_{C}$ denote their number. $n_s$ denotes the largest window, in the worst case, $n_{C}=|D|, n_{R}=\left \lfloor{n/d_{min}}\right \rfloor, n_{s}=n$.
Overall, since we limit the number of iterations to a constant hyperparameter in practice, we obtain $\mathcal O(n^2 + |V|^3n^3 +(n_{R}^2+n_{C}^2)n_{TD}^3)$. We will include this in the revised manuscript.

\paragraph{Parameters} 
Our method has only two hyperparameters, minimum regime length $d_{min}$, and the maximum lag between a cause and its effect $\mathbf \tau$. Our competitors need similar parameters. If $d_{min}$ is set lower value than the actual minimum regime length, our method will in addition to the true changepoints likely return additional spurious changepoints. As long as $d_min$ is not set too low (i.e. that we can no longer estimate the functions well) the partitioning will assign each of these `slices' to the same regime. 
Similarly, as long as $\mathbf \tau$ is chosen higher or equal to the true value, the edge corresponding to the correct time lag will always have a higher score than the others (given pure regimes and contexts).
We will include an experimental sensitivity analysis of these parameters in the Appendix.
\paragraph{Algorithm} Here, $\mathbf X^d_t$ (first defined on page 2) denotes the whole time series with all datasets over all time indices in $\mathcal{T}$ taken by the algorithm as input. Thus, the context partition is indeed done over all datasets. We can modify this notation to e.g. $\mathbf X^D_\mathcal{T}$ to avoid confusion.
\paragraph{Code} We will make our Python implementation publicly available. 

% Thank you for your detailed comments. 

% **Problem setting** Yes, our approach allows multiple variables to change at the same time. We set a changepoint $l \in \mathcal L$ whenever *at least* one node $i$ changes at $l$, but the output of our method will show which variable sets change at which locations. We will clarify this in the problem-setting section.

% **Complexity** We inherit the complexities of the chosen components, namely PELT in $\mathcal O(n^2)$, where $n=|\mathcal T|$; Causal Discovery in $\mathcal O({n_V}^3)$ (Mian et al. 2021) for $n_V$ nodes, together with GP regression in $\mathcal O({n_{s}}^3)$ for $n_{s}$ samples;
% and partitioning in $O(({n_{R}}^2+{n_{C}}^2){n_{TD}}^3)$ as the kernel test is applied to pairs of regimes and contexts, where $n_{R},n_{C}$ denote their number. $n_s$ denotes the largest window, in the worst case, $n_{C}=|D|, n_{R}=\left \lfloor{n/d_{min}}\right \rfloor, n_{s}=n$.
% Overall, since we limit the number of iterations to a constant hyperparameter in practice, we obtain $\mathcal O(n^2 + |V|^3n^3 +({n_{R}}^2+{n_{C}}^2){n_{TD}}^3)$. We will include this in the revised manuscript.

% **Parameters**
% Our method has only two hyperparameters, minimum regime length $d_{min}$, and the maximum lag between a cause and its effect $\tau_{max}$ (bold $\tau$ in the paper). Our competitors need similar parameters. If $d_{min}$ is set lower value than the actual minimum regime length, our method will in addition to the true changepoints likely return additional spurious changepoints. As long as $d_{min}$ is not set too low (i.e. that we can no longer estimate the functions well) the partitioning will assign each of these "slices" to the same regime. 
% Similarly, as long as $\tau_{max}$ is chosen higher or equal to the true value, the edge corresponding to the correct time lag will always have a higher score than the others (given pure regimes and contexts).
% We will include an experimental sensitivity analysis of these parameters in the Appendix.

% **Algorithm** Here, $\mathbf X^d_t$ (first defined on page 2) denotes the whole time series with all datasets over all time indices in $\mathcal{T}$ taken by the algorithm as input. Thus, the context partition is indeed done over all datasets. We can modify this notation to e.g. $\mathbf X^D_\mathcal{T}$ to avoid confusion.

% **Code** We will make our Python implementation publicly available.

\section{Reviewer 3}
Thank you for your response and suggestions. 
\paragraph{Repeating Edge Property}
The repeating edge property, though sometimes going by other names such as causal stationarity, is a very common assumption in time series causal discovery since it allows us to discover a window causal graph over a finite number of nodes, as opposed to the entire time series graph over (in principle) an infinite number of nodes.

Assuming that edge directions do not change and that edges do not vanish seems reasonable to us for a wide range of applications, as many systems are governed by physical principles, well-established social behaviors, or invariant biological processes. For instance, in the Drivers of River Discharge case study, there is a physical link between precipitation and the subsequent river discharge, making this edge persist in time. Changes in edge strength, such as due to seasonal effects, are however possible and also realistic. 
Other examples where this assumption is reasonable include considering the effect of a drug on metabolism, where the strength of the effect may vary among individuals but the delay of the effect is due to the blood flow velocity, or changes in trade market conditions, where the delay is constrained by the frequency of the financial reports.
We will include a discussion on our assumption in the manuscript if it is insightful.
\paragraph{Edge-Greedy Search} Indeed. The method we base our search algorithm on, Globe (Mian et al, 2021), is very efficient, returns fully oriented causal graphs, and even though it comes with guarantees only for trees, performs very well in practice in recovering arbitrary DAGs. It will make for interesting future work to replace it with an algorithm that comes with stronger guarantees.

% Thank you for your response and suggestions. 

% **Repeating Edge Property**
% The repeating edge property, though sometimes going by other names such as causal stationarity, is a very common assumption in time series causal discovery since it allows us to discover a window causal graph over a finite number of nodes, as opposed to the entire time series graph over (in principle) an infinite number of nodes.

% Assuming that edge directions do not change and that edges do not vanish seems reasonable to us for a wide range of applications, as many systems are governed by physical principles, well-established social behaviors, or invariant biological processes. For instance, in the Drivers of River Discharge case study, there is a physical link between precipitation and the subsequent river discharge, making this edge persist in time. Changes in edge strength, such as due to seasonal effects, are however possible and also realistic. 
% Other examples where this assumption is reasonable include considering the effect of a drug on metabolism, where the strength of the effect may vary among individuals but the delay of the effect is due to the blood flow velocity, or changes in trade market conditions, where the delay is constrained by the frequency of the financial reports.
% We will include a discussion on our assumption in the manuscript if it is insightful.

% **Edge-Greedy Search** Indeed. The method we base our search algorithm on, Globe (Mian et al, 2021), is very efficient, returns fully oriented causal graphs, and even though it comes with guarantees only for trees, performs very well in practice in recovering arbitrary DAGs. It will make for interesting future work to replace it with an algorithm that comes with stronger guarantees.

\subsection{Details to Individual Points}
\subsection{Reviever 1}
\subsubsection{Notation}
\begin{itemize}
\item Q3. We set the maximum time lag to $\mathbf \tau=2$ in our experiments. 
\item Q4. Yes, we overload notation here and refer to a deterministic function $\mathcal C$ so that $C(d) = c$ assigns a dataset $d$ to a single context $d$. We are open to remove this notation if it leads to confusion and otherwise will define it clearly in the manuscript. 
\item Q5. $X^d_t$ is one sample of variable $i$ at time $t$ in dataset $d$, making the parent set well defined. Hereby and similarly for the functions $f^{k,r}_{(i)}$, we omitted the index $i$ to avoid clutter, but we agree that they should be included for conciseness. 
\item Q6. Correct, thanks for pointing this out.
\item Q9. We will add subscripts $f^{k,r}_{(i)}, f^{k,r}_{(j)}$ to clearly refer to the functions corresponding to $X_{(i)}, X_{(j)}.$
\item Q13. Typo
\end{itemize} 


\subsubsection{Questions}
\begin{itemize}
\item  Q1. In Definition 3 we assume that there is a single, fixed set $\mathcal L$ of regime changepoints common in all contexts (for instance, when the source of non-stationarity is a seasonal trend that applies in all contexts).
\item  Q2. Not all causal relations are assumed to be invariant, as non-stationarity arises from changes in the functions $f^{k,r}_{(i)}$ for some $k,r,i$. They remain invariant across time in a regime (and across datasets in a context). We specified this in the functional modeling Assumption 3 but we can make this explicit in another assumption if it is helpful. 
\item  Q7. In our simulations, we found small values $s=30$ to be effective  to detect regime shifts. 
\item  Q8. \emph{Computational complexity}
\item  Q10 Assumption 8 in the supplement corresponds to Assumption 2, we will ensure consistent numbering. Assumption 7 introduces an alternative formulation. 
\item  Q11  Independence of $Z_i, Z_j$ means that the values $P(Z_i=r)$ of these discrete variables (for example, shown as the colored regions in Fig. 1)  are assigned independently. 
\item Q12 \emph{Efficiency sample size for regime and context partitioning.} 
We inherit the sample efficiency of the kernel discrepancy test. 
\item Q14  
The true noise distribution doesn't change between regimes, but when the regime changes, the residuals computed using the function corresponding to the former regime do not correspond to the true noise anymore. This is how we can detect regime changes.
\item Q15 Regarding the independence test for the regime and context partitioning: non-IDDness might create a spurious dependence to the auxiliary variable because the samples within a time interval are correlated. 
It is an additional justification for having a $d_{min}$ since the correlation will exist within samples close in time but not with the others. 
The risk here is to get more distinct regimes than needed, but each sample will have a causal mechanism fitted with datapoints from its true regime, while the opposite would be much worse.
Regarding the DAG search?
\item Q16 \emph{taumax and large parent sets.} A large $\tau_{max}$ does not necessarily imply a large parent set, but increases the number of candidates. There is a computational impact on the DAG search as its complexity relies on the number of nodes in the DAG.
\item Q17 We adapted the code base for JPCMI, which is publicly available in the TIGRAMITE Python package, as follows. The code base already allows generating data  with ground truth contemporaneous and lagged links in multiple contexts. We generate multiple regimes as follows (...)
\item Q18 While we are not sure about convergence guarantees our simulation results strongly indicate that we need only few iterations for convergence. In particular, in difference to R-PCMCI our algorithm converged in all experiments. 
As a starting point, we use an empty DAG and look for changepoints in the raw data instead of residuals. Some of the changepoints might be obvious and directly detected. Not all variables are intervened on at each regime change, we assume that for most nodes, the function fitted overall data with the correct set of parents will still be better in the causal direction than in the anti-causal direction. Then, having the correct changepoints will improve the parent identification (partially based on the partitions), which will improve the changepoint detection (based on the parents).
\item Q19 \emph{Details on how the baselines were applied to multiple datasets.}
\item Q20 \emph{Include table of experiment with larger sample size.}
\end{itemize}
 

\section{Reviewer 2}
\begin{itemize}
\item Q1. Yes, there is a change for at least one variable but there can be more. We can clarify this point in the problem setting section.  %Can the proposed model allow the temporal (or spatial) changes from two or more variables over T (or D)? Can the method find which variable induces the temporal or spatial changes? It seems not very clear from the problem setting.
\item Q2. Changepoint detection (PELT): $\mathcal O(|T|^2)$ in worst cases, as it is applied to $|T|$ samples (and to all variables and datasets jointly). GLOBE (original version): $\mathcal O(|V|^3)$, Gaussian process regression over $n$ samples: $\mathcal O(n^3)$,
regime and context partitioning: $O(|R||C|d_{max}^3)$ because we apply the kernel test ($O(n^3)$ complexity I believe) to all pairs of regimes $|R|$ and contexts $|C|$, with $d_{max}$ the maximum number of samples. When $|R|$ and $|C|$ are not fixed, this would be $|T||D|(|T|+|D|)^3$ (probably something smaller?)
Overall, if we limit the number of iterations to a constant $\lambda_c,$ we obtain $\mathcal O(|T|^2 + |V|^3(|T|+|D|)^3 + |T||D|(|T|+|D|)^3)$.
%From Eq.(2), the authors optimize iteratively G_t, L, C and R. It looks like a more complicated optimization procedure than usual. It would be good to discuss the computational complexity. How many parameters are to be tuned? It would be good to see the sensitivity analysis of those parameters, e.g., d_min, tau, etc. 
\item Q3. $\mathbf X^d_t$ (first defined on page 2) denotes the whole time series with all datasets over all time indices in $\mathcal{T}$ taken by the algorithm as input. Thus, the context partition is done over all datasets. %From lines 4-6 of Algorithm 1, it seems strange to only use the dth dataset to learn the contexts C, since the context changes exist in multiple datasets. Did I misunderstand something?
\item Q4. The code will be made publicly available on the authors' website and provided alongside the revised manuscript. %The code is not available.
\end{itemize}

\section{Reviewer 3}
\begin{itemize}
\item Q1. The assumption that the edge direction won't change and that no edge will disappear seems reasonable to us for a wide range of applications, as many systems are governed by physical principles, well-established social behaviors, or invariant biological processes. For instance, in the Drivers of River Discharge study case, there is a physical link between the precipitations and the subsequent river discharge, making this edge constant. The repeating edge property is a stronger assumption when considering the variability in time lag. It is already a strong assumption when considering stationary time series, as noise could induce variability in delay. Increasing the time step between two measurements can help mitigate this. 
When considering different contexts and regimes, the mechanism changes can in fact cover these variations, for instance via a coefficient that modifies the rate at which the effect is observable. 
Examples where this assumption is reasonable include considering the effect of a drug on a metabolism, where the strength of the effect may vary among individuals but the delay of the effect is due to the blood flow velocity, or changes in trade market conditions where the delay is constraint by the frequency of the financial reports.
%but it is necessary to  If assumption violation, the information flows through the auto-correlation. If different time-lag for different regimes, ? Time lag could also vary within a regime. using a higher time step can help reduce the impact of noise. If assumption removed, we can't have multiple measurements, only a full temporal causal graph can represent the data. %Can you provide some examples that you expect the assumptions to be reasonable, especially for Assumption 2 (repeating edge property)? It looks like a strong assumption since it require some causal relaionship to always hold for a fix amount of time gap.
\item Q2. anything in GLOBE paper? 
This is a valid point. While our scoring function is consistent, the causal graph search may not provably recover the ground truth due to its edge-greedy nature, that is, consideration of pair-wise edges. 
We opt for a greedy search because the results from Mian et. al. for i.i.d. continuous data, and our own simulations with time series data, suggest a strong performance in practice.
An interesting line of future work would be to develop a score-based method that provably identifies the causal graph efficiently. 
%Is there any provable guarantees that the solution learned by you algorithm is close to the ground-truth? In particular, I'm concerned about whether the edge-greedy search in algorithm 1, line 5 can actually recover the true causal graph.
\end{itemize}
